Toxicity Detection is NOT all you Need: Measuring the Gaps to Supporting Volunteer Content Moderators

Extensive efforts in automated approaches for content moderation have been focused on developing models to identify toxic, offensive, and hateful content with the aim of lightening the load for moderators. Yet, it remains uncertain whether improvements on those tasks have truly addressed moderators' needs in accomplishing their work. In this paper, we surface gaps between past research efforts that have aimed to provide automation for aspects of content moderation and the needs of volunteer content moderators, regarding identifying violations of various moderation rules. To do so, we conduct a model review on Hugging Face to reveal the availability of models to cover various moderation rules and guidelines from three exemplar forums. We further put state-of-the-art LLMs to the test, evaluating how well these models perform in flagging violations of platform rules from one particular forum. Finally, we conduct a user survey study with volunteer moderators to gain insight into their perspectives on useful moderation models. Overall, we observe a non-trivial gap, as missing developed models and LLMs exhibit moderate to low performance on a significant portion of the rules. Moderators' reports provide guides for future work on developing moderation assistant models.

==> sections/method.tex <==
To assess the gap between the current models on content moderation and the models needed to satisfy the various sets of moderation rules, we conduct a model review on Hugging Face and test the state-of-art LLMs. 
The model review intends to inform us of the progress of past research works on covering the moderation rules. 
Meanwhile, the model test reveals the SOTA model's performance in detecting violations of these rules.

\subsection{Hugging Face Model Review}
Different from a literature review, a model review directly reveals what NLP models are publicly available that can be adapted to assist content moderators in making moderation decisions.    
We thus conduct a model review via Hugging Face (HF)\footnote{\url{https://huggingface.co/models}}, which is an open-source platform that provides pre-trained models for various NLP tasks, to understand the progress of existing research on covering various moderation rules. In this work, we focus on Reddit\footnote{\url{https://www.reddit.com/}} rules. 
To conduct the model review, we gather rules from three subreddits and manually annotate each rule to assess whether there exists an HF model suitable for detecting such rule violations. 

\paragraph{Subreddit Rules Collection}
\citet{Chandrasekharan_2018} clustered 100 subreddits into six Meso groups plus four Micro groups based on similarity of the removed comments. 
We pick three subreddits -- \textit{r/Atheism, r/Movies, r/AskHistorian}, from three of the Meso subreddit clusters and use their rules as representations for study. 
We verify the coverage of the three subreddits' rules by cross-referencing them with the list of $25$ rule types aggregated from 1000 subreddits by \citet{Fiesler_2018}. We ensure that all text-based rule types are covered by at least one of the rules from the three subreddits. See appendix \autoref{tab:rule_types} for our list of rules and its cross-referencing with the list of rule types.

\paragraph{Annotation Procedure}
For each rule, we crawl its rule description from Reddit. Based on the rule descriptions, we find keywords for model searching on HF. For example, for the rule \texttt{Personal Attacks or Flaming --- ``Keep things civil. Avoid fighting words and personal attacks. (applies to all forms of user content, including the user's name.)''}, we use keywords \texttt{doxxing, cyberbullying}. We then search on HF by matching keywords with model names or model cards to find the model that is most relevant to each moderation rule. 
We traverse the top 20 search results to find the most matching model. If nothing relevant is found, we declare there is no matching model for this moderation rule. We also skip any model that does not contain a model card (i.e., no model description). See appendix (TODO) for the keywords we used and the matching models for each rule.

\begin{table}
\centering
\footnotesize
\rowcolors{2}{gray!25}{white}
\begin{tabular}{l@{~~~}p{5.6cm}}
\hline 
\rowcolor{gray!50}
 \textbf{Label}& \textbf{Annotation Question} \\ \hline
\Qrule & Can detection of violations on this rule be done by rule-based approaches, e.g. RegEx?\\
\Qhate & Is this rule covered by hate-speech or toxicity detection?\\
\Qmatch  & Is there an HF model that can be used to detect violations of this rule?\\
\Qpurpose & What is the original purpose of this matching model?\\
\Qgap & In order to adapt this model to detect violations of this rule, what needs to be adjusted?\\
\hline
\end{tabular}
\caption{\label{tab:anno_q} Model review annotation questions.\vspace{-1em}}
\end{table}

With the matching model, we then annotate each moderation rule with the annotation questions, as listed in \autoref{tab:anno_q}.

\noindent~~$\blacktriangleright$~\Qrule: we first mark out the rules that can easily be handled by rule-based approaches, such as detecting reposts. The possible answer to this question is \textit{yes} or \textit{no}. 

\noindent~~$\blacktriangleright$~\Qhate: to understand what portion of the policies are related to toxicity detection, we mark the rules that can be handled by toxicity detectors, such as detecting harassment. Possible answers are \textit{yes} or \textit{no}. 

\noindent~~$\blacktriangleright$~\Qmatch: as described above, we search on HF to find a matching model for each rule if the rule cannot be handled by rule-based approaches. We then decide whether the model can be used for this rule. Possible answers are \textit{yes}, \textit{yes, but with changes to the model} or \textit{no}. 

\noindent~~$\blacktriangleright$~\Qpurpose: for the record, we also note the intended use case for the model as claimed in the model card.

\noindent~~$\blacktriangleright$~\Qgap: finally, we write the changes, if needed, for the model to be used for this rule, such as domain adaptation.


\subsection{LLMs Performance on SubReddit Rules}
Finding a suitable NLP model for handling a moderation rule is not trivial, let alone executing the necessary modifications to the model, and some rules simply lack a matching model to address their specific issues. It requires familiarity with NLP techniques and tasks, which may not be within the scope of a content moderator's abilities.
The question-answering-based LLM applications, on the other hand, are more practical for content moderators to employ in assisting their jobs. 
Therefore, we also evaluate the LLMs' performance in catching rule-violating comments.
For this evaluation, we focus on the \textit{r/AskHistorian} subreddit and two LLMs -- Llama-2\footnote{\url{https://huggingface.co/meta-llama/Llama-2-13b-hf}}~\cite{llama2} and GPT-3.5 \trista{how to cite?}. 

\paragraph{Evaluation Dataset \trista{or Test Dataset?}}
Supported by \trista{one of the authors, who is also [can we say this?]} a volunteer moderator on \textit{r/AskHistorian}, we crawled $TODO$ questions and $TODO$ comments from the \textit{r/AskHistorian} subreddit. Each question and comment is also marked with the rule it violated. Note that the questions and comments may violate multiple rules, but only the most severe one is marked here. We also crawled $TODO$ questions and comments that do not violate any \textit{r/AskHistorian} rules. We use these crawled data as our evaluation dataset\footnote{The dataset will be published after the anonymity period.}.

\paragraph{Model Testing and Prompts}
For GPT-3.5, we test the model's performance in a zero-shot context. 
We experimented with various methods of prompting the model, and here is the most effective prompt we discovered.
\begin{displayquote}
    \texttt{You are a moderator assistant.}\\
    \texttt{There is a moderation rule named \{rule\} that says \{rule description\} Does the following content violate the \{rule\} rule? Just answer yes or no.}\\
    \texttt{\{test content\}}
    
\end{displayquote}

\noindent For Llama-2, we test the model in a few-shot context. For question contents, we provide the model with three examples that violated the rule and three examples that did not. For comment contents, we provide one example for each due to the model's input length limit. See appendix (TODO) for the exact prompt we use for Llama-2. 

==> sections/result.tex <==
\begin{figure*}[t]
    \centering
\includegraphics[width=0.75\columnwidth,angle=90,clip=true,trim=250 0 50 0]{sections/HF_results.pdf}
    \caption{xxx}
    \label{fig:HF-results}
\end{figure*}


\subsection{Model Review Results}
As shown in TODO, among the $41$ moderation rules, most of the rules ($90\%$) can not be handled by rule-based approaches. Among the $90\%$, only $19\%$ are toxicity-related rules. This reemphasizes that models solely designed for detecting toxic content fall short in meeting the practical needs of content moderators.


Among the not-toxic-related rules, only $20\%$ has a HF model that can be used directly to moderate for this rule. A vast majority of the rules $43\%$ requires some model modifications in order to be adapted for the rule, whereas $37\%$ has no matching model at all. These rules include: xx,xx,xx,....
On the other hand, among the toxic-related rules, we see that the majority of the rules $57\%$ require model modifications. 
This indicates 


Among the model changes, we find there are mostly four kinds.  
Detailed annotations for each moderation rule is presented in the appendix TODO.


\begin{figure*}[t]
    \centering
\includegraphics[width=1.2\columnwidth,angle=-90,clip=true,trim=0 0 50 0]{sections/Model-Questions.pdf}
    \caption{xxx}
    \label{fig:model-question}
\end{figure*}

\begin{figure*}[t]
    \centering
\includegraphics[width=1.3\columnwidth,angle=-90,clip=true,trim=0 0 0 0]{sections/Model-Comments.pdf}
    \caption{xxx}
    \label{fig:model-comment}
\end{figure*}
